Secure Full Duplex Integrated Sensing and Communications

The following paper models a secure full duplex (FD) integrated sensing and communication (ISAC) scenario, where malicious eavesdroppers aim at intercepting the downlink (DL) as well as the uplink (UL) information exchanged between the dual functional radar and communication (DFRC) base station (BS) and a set of communication users. The DFRC BS, on the other hand, aims at illuminating radar beams at the eavesdroppers in order to sense their physical parameters, while maintaining high UL/DL secrecy rates. Based on the proposed model, we formulate a power efficient secure ISAC optimization framework design, which is intended to guarantee both UL and DL secrecy rates requirements, while illuminating radar beams towards eavesdroppers. The framework exploits artificial noise (AN) generation at the DFRC BS, along with UL/DL beamforming design and UL power allocation. We propose a beamforming design solution to the secure ISAC optimization problem. Finally, we corroborate our findings via simulation results and demonstrate the feasibility, as well as the superiority of the proposed algorithm, under different situations. We also reveal insightful trade-offs achieved by our approach.

==> Actions/DFRC-tests-for-eve.tex <==
The \ac{DFRC} \ac{BS} also aims to test for presence/absence of target eavesdroppers that are possibly located at angles $\theta_1 \ldots \theta_P$ with respect to the \ac{DFRC} \ac{BS}, respectively. 

==> Actions/DongDongLi-work.tex <==
The work in \cite{9927490,10039359} models a physical layer security \ac{NOMA}-aided \ac{ISAC} system, which exploits \ac{AN}. In particular, a secure precoding approach was designed by maximizing the sum secrecy rate for different users through artificial jamming, and simultaneously utilizing the \ac{NOMA} signals for target detection.

==> Actions/Problem1o3_copy.tex <==
\textcolor{blue}{
\begin{equation}
 \label{eq:problem1_3_copy}
\begin{aligned}
(\mathcal{P}_{1.3}^{(m)}):
\begin{cases}
\min\limits_{\big\lbrace \substack{     \pmb{V}_1 \ldots \pmb{V}_L, \\ 
									 \pmb{W}, 
									  \pmb{p} }  \big\rbrace}&   \sum\nolimits_{\ell = 1}^L\trace(\pmb{\pmb{V}}_\ell) + \trace(\pmb{W}) + \pmb{1}^T \pmb{p} \\
\textrm{s.t.}
 &  \frac{1}{\zeta_{\ell}^{\tt{DL}}}
	\trace(\pmb{V}_\ell\pmb{H}_{r,\ell})
	- \Big(\sum\limits_{\substack{k = 1  }}^K p_k \vert q_{k,\ell} \vert^2 +\sum\nolimits_{\substack{ \ell^{'} \neq \ell}} \trace(\pmb{V}_{\ell'}\pmb{H}_{r,\ell}) + 
	\trace(\pmb{W}\pmb{H}_{r,\ell})  +
	\sigma_{\ell}^2
	\Big)
	\geq 0, \quad \forall \ell= 1 \ldots L, \\
&  
	\frac{\zeta_{k}^{\tt{UL}}}{p_k}
	  +
	  \pmb{h}^H_{t,k}
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{\Phi}_k
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{h}_{t,k}
	-
	2  \pmb{h}^H_{t,k}
	[\pmb{\Phi}_k^{(m)}]^{-1}
	 \pmb{h}_{t,k} \leq 0
, \quad \forall k  = 1\ldots K, \\
&  	\frac{1}{\zeta_{p,\tt{DFRC}}^{\tt{Eve}} }
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\Big( \sum\limits_{\ell = 1}^L \pmb{V}_\ell \Big)\pmb{a}_{N_T}(\theta_p)
	  \leq 
	\sum\limits_{\substack{k = 1  }}^K p_k \vert g_{k,p} \vert^2 + 
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2 , \quad \forall p = 1\ldots P \\
&  \frac{1}{\zeta_{p,k}^{\tt{Eve}} }
	p_k \vert g_{k,p} \vert^2 
	-
	\Big(
	\sum\nolimits_{\substack{ k' \neq k }} p_{k'} \vert g_{k',p} \vert^2 + \vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{Q}\pmb{a}_{N_T}(\theta_p) + \sigma_p^2
	\Big) \leq 0 , \quad \forall p= 1\ldots P, \ k= 1\ldots K \\
& \trace\Big( (\sum\nolimits_{\ell = 1}^L\pmb{V}_\ell
	+
	\pmb{W}) \pmb{A}_s \Big) \leq \ISMR_{\tt{max}} \times \trace\Big( (\sum\nolimits_{\ell = 1}^L\pmb{V}_\ell
	+
	\pmb{W}) \pmb{A}_m \Big) , \\
 & \pmb{W} \succeq \pmb{0},  \ \pmb{p} \succeq \pmb{0},\ \pmb{V}_\ell \succeq \pmb{0}, \quad \forall \ell= 1\ldots L.  \\
\end{cases}
\end{aligned}
\end{equation}
}

==> Actions/imperfect-csi-contribution.tex <==
\textbf{Imperfect \ac{CSI}-aware Design for \ac{FD} \ac{ISAC} power minimization.} To account for \ac{CSI} errors that arise due to channel estimation errors and outdated effects, we devise a \ac{BCCD} iterative algorithm to solve an extended robust/perturbed version of the secure \ac{ISAC} optimization problem.

==> Actions/summary-of-actions.tex <==
In light of the reviewers comments, we summarize our action items as follows:
\begin{itemize}
%% R1
\item We have now emphasized the new technical challenges arising in the proposed \ac{FD} \ac{ISAC} setting from a security point of view, and compared with \cite{10158711} and \cite{10159012} in order to highlight the contributions and major differences with these works.
 \item We have added explanations on why we have resorted to \ac{ISMR} optimization. In short, we have highlighted two main points: 1) As we assume knowledge of eavesdropper \acp{AoA} and through optimizing the \ac{ISMR}, we also indirectly improve further localization performance, e.g. delay and doppler estimation, so as to reliably estimate the absolute position of the eavesdroppers. In addition, the ISMR further allows us to track the eavesdroppers by utilizing the reliably estimated delay and doppler information, and accurately steering the mainlobe beams defined by the ISMR. 2) The ISMR allows us to adjust the mainlobes reliably to account for any \ac{AoA} uncertainty on the eavesdroppers. 
 \item We have now checked and corrected equation \eqref{eq:constraint38} (previously equation (38)) in the revised manuscript. In addition, we have verified that this particular constraint is convex, and added the justification.
 \item We have now double checked the proof and as the previous constraint remains convex, the proof still holds. Some necessary amendments and modifications have been done and we have corrected some typos in the proof and corrected some missing statements. 
\item We have mentioned additional security issues following \cite{10024766} and references therein. In addition, we have indicated how deep learning methods can be useful for future wireless communications. Moreover, we have indicated how \ac{EL} in particular can be used to distribute the implementation of \ac{DL} methods among several edge devices, which can in turn reduce the computational complexity, as well as reduce the dangers of malicious attacks due to the distributive nature. 
\item We went through the article again to correct typos, improve text and change the format of the figures in order to make them more clear and appealing. 
%% R2
\item We have indicated that our model does not separate the sensing and communication signals, where both are integrated within the same signal. In addition, due to clutter presence, we have clarified that a portion of the \ac{DL} signal can scatter from clutter to the \ac{DL} users. Moreover,  we also highlighted that the \ac{UL} channels also account for clutter, as part of the channel propagates towards clutter then back to the \ac{DFRC} \ac{BS}.
\item We have improved the introduction by including some recent work especially those by Dongdong Li \cite{9927490}, \cite{10039359}. In addition, we have added more existing work, as well as rewriting several statements.
\item We now clarify that downlink and uplink users are  single-antenna users.
\item We now integrate the {\tt{acronym}} package of {\LaTeX} to ensure that all acronyms are properly abbreviated. For example, we use the acronym SI which automatically replaces each occurrence of 'self interference'.
\item We have now bolded different keywords appearing in Algorithm 1, such as \textbf{input}, \textbf{while}, \textbf{for} and other statements.
\item As we have redone the simulations, we have now appropriately reduced the number of numerical points so as to make the curve trend clearer within the figures.
\item We have indicated the units of $\sigma_n^2$, $\sigma_p^2$, $\sigma_\ell^2$, $\zeta^{\tt{UL}}$ and $\zeta^{\tt{DL}}$ within the figures as well as the text.
\item We have now unified the format of the references. More specifically, we now use {\tt{BibTeX}} with the latest {\tt{IEEEtran.bst}} version in order to guarantee that all references follow the same format.
%% R3
\item In this response letter, we have described a framework that extends this work to the case of imperfect \ac{CSI}, by utilizing ellipsoidal uncertainties on the \ac{CSI} vectors. Furthermore, in this response letter, we have designed a \ac{BCCD} method to solve the resulting imperfect \ac{CSI} optimization problem. Due to the lack of space in the manuscript, we have mentioned in the updated manuscript that this extension to imperfect \ac{CSI} will be part of our future work.
\item We have indicated that the \acp{AoA} of the eavesdroppers are known to the \ac{DFRC} \ac{BS} and clarified that the \ac{DFRC} \ac{BS} estimates them from a previous stage. Moreover, we have mentioned that the \ac{DFRC} \ac{BS} is further interested in estimating additional sensing parameters such as the delay and doppler parameters through the received signal at the \ac{DFRC} \ac{BS}. Also, we have mentioned \ac{ISAC} works that assume knowledge of target \acp{AoA}.
\item We have provided a reference for the \ac{SI} channel model in eq. \eqref{eq:SI} of the updated manuscript (previously equation (8)).
\item We have clarified how the problem in equation  \eqref{eq:problem1} (previously equation (27)) can be reformulated as that in \eqref{eq:problem1_1} (previously equation (28)).
\item We have provided more information on how the comparisons between full-duplex and half-duplex modes are done.
\item We have repeated our entire simulations in order to make a wide applicability of the proposed \ac{FD} \ac{ISAC} model and the proposed algorithm. In particular, we have referred to \cite{8207426} in order to set up a practical simulation environment that describes a typical \ac{mmWave} communication model. The new simulation environment also sets the UL/DL and eavesdroppers at certain positions and takes into account small-scale fading and large-scale fading, which includes pathloss and shadowing. Moreover, we have studied through simulations the performance under different channel conditions such as Rayleigh and Rician. 
%% R4
\item We have now added \ac{UL}-to-\ac{DL} interference to the $\ell$-th legitimate receiver, the same way it was added to the $p^{th}$ eavesdropper. Therefore, all \ac{DL} users, as well as eavesdroppers receive the signals from the \ac{UL}.
Therefore, equation \eqref{eq:DL-signal-2} (in the updated manuscript) has now included the \ac{UL}-to-\ac{DL} interference, in a similar spirit that \eqref{eq:pth-eve} (in the updated manuscript) accounts for it.
As a result, many major changes have been done, including changes to the proposed secure \ac{FD} \ac{ISAC} optimization problem which now accounts for this \ac{UL}-to-\ac{DL} interference and the algorithm which is now adapted accordingly.
We have also repeated the simulations taking into account this \ac{UL}-to-\ac{DL} interference.
Furthermore, we have highlighted the difference between \eqref{eq:DL-signal-2} and \eqref{eq:pth-eve}. In particular, we regard eavesdroppers as radar targets, where a strong and dominant \ac{LoS} component exists between the \ac{DFRC} and the eavesdroppers, which is applicable to \ac{UAV}-type applications \cite{10098686}.
\item We now clarify the choice of different values of noise power level in accordance with reference \cite{8207426}. The noise power levels are now reasonable. 
Since pathloss/shadowing are part of the simulation flow, $-80\dBm$ for noise power is typically acceptable, as the pathloss between \ac{DFRC} \ac{BS} and \ac{DL} is of the order of $-60\dBm$ with the given parameters, hence an \ac{SNR} of the order of $20\dB$, which is typical \cite{8207426}.
\item We now compare the optimized proposed system with/without AN in particular in Fig. \ref{fig:tradeoff2} of the updated manuscript. We have seen significant gains when introducing AN in terms of total power consumed to achieve a fixed secrecy rate. In addition, there are significant gains when introducing AN in terms of feasibility rate of the proposed optimization problem.
\item We have clarified how the competing schemes are optimized and in what sense they are optimized. We have added an optimized scheme to compare with which is the proposed scheme but without AN. In addition, we now clarify why the system with AN can achieve higher secrecy rate in certain points where the eavesdroppers are experiencing high noise levels. 
\item All other minor comments of the reviewers have been addressed.
\end{itemize}

==> Actions/target-abscent-present-gammap.tex <==
Note that if the $p^{th}$ eavesdropper is absent, then $\gamma_p = 0$. 

==> Actions/unknown-eve-locations.tex <==
The locations of the eavesdroppers are assumed to be unknown, and the \ac{DFRC} \ac{BS} wishes to illuminate beams towards locations to maximize its detection capabilities while probing for multi-target detection\cite{7849236}, and minimizing the communication information exposed in these directions.
For simplicity, we assume that eavesdropping targets are present and that multi-target detection\cite{7849236} is performed at a later stage.
In addition, the \ac{DFRC} \ac{BS} can infer additional sensing information from the eavesdropping targets, such as speed, distance and \ac{RCS}.


==> Actions2/summary-of-actions.tex <==
In response to the comments from the Associate Editor and reviewers, we outline our action items as follows:
\begin{itemize}
\item We restructured the final part of Section I.A to enhance the coherence of existing work. Specifically, we relocated the content associated with references [25], [26], [27] after the introduction of ISAC. Additionally, we unified the explanations about Ref [25] into a single sentence.
\item A brief description of the FD operation has been incorporated into the Introduction, directly after the mentioning FD.
\item Extra equations have been added below equation (3) to elucidate the \ac{mmWave} communication channel model of $\pmb{h}_{r,l}$.
\item The text following equation (4) has been revised to accurately depict the first four terms.
\item The symbol rho is now used to describe terms related to rate, while zeta reflects SINR terms.
\item The cell radius has been adjusted to $200\meters$ based on the maximum location of users at that distance.
\item References for the Rayleigh fading mmWave channel and a cell radius of $500\meters$ have been provided.
\item Assumptions for simulations in Section V.A have been explicitly mentioned.
\item Further elaboration on vector $\pmb{w}$ has been included, emphasizing its role not only in AN generation but also in enhancing sensing performance.
\end{itemize}


==> Equations/steering-vector-copy-2.tex <==
	\label{eq:steering-vector-copy-2}
	\pmb{a}_{N_T}(\theta)
	&=
	\begin{bmatrix}
		a_1(\theta) & \ldots & a_{N_T}(\theta) 
	\end{bmatrix}^T, \\
	\label{eq:steering-vector-2-copy-2}
	\pmb{a}_{N_R}(\theta)
	&=
	\begin{bmatrix}
		a_1(\theta) & \ldots & a_{N_R}(\theta) 
	\end{bmatrix}^T.

==> Equations/steering-vector-copy.tex <==
	\label{eq:steering-vector-copy}
	\pmb{a}_{N_T}(\theta)
	&=
	\begin{bmatrix}
		a_1(\theta) & \ldots & a_{N_T}(\theta) 
	\end{bmatrix}^T, \\
	\label{eq:steering-vector-2-copy}
	\pmb{a}_{N_R}(\theta)
	&=
	\begin{bmatrix}
		a_1(\theta) & \ldots & a_{N_R}(\theta) 
	\end{bmatrix}^T.

==> Response/DongDongLi-response.tex <==
The authors would like to thank the reviewer for the comment, and for bringing to our attention the mentioned works. 
We have cited and discussed the work of Dongdong Li on secure \ac{NOMA} \ac{ISAC}, namely \cite{9927490} and its earlier version \cite{10039359}.
We have also enriched the Introduction with additional latest work on \ac{ISAC}.

==> Response/Equivalence-between-two-problems.tex <==
The authors would like to thank the reviewer for the comment.
The first constraint appearing in problem $(\mathcal{P}_1)$ within equation \eqref{eq:problem1} of the revised manuscript is
\begin{equation}
	\SR_{\tt{DL}} \geq \zeta^{\tt{DL}},
\end{equation}
which, by utilizing the definition of the worst-case secrecy rate in the \ac{DL} via equation \eqref{eq:SR_DL} of the revised manuscript, is equivalent to 
\begin{equation}
		\min_{\ell,p}
\Big[
\log_2(1+\SINR_{\ell}^{\tt{DL}})
-
\log_2(1+\SINR_{p,\tt{DFRC}}^{\tt{Eve}})
\Big]^+
\geq
 \zeta^{\tt{DL}}.
\end{equation}
Now we define $LP$ positive lower-bounds, i.e. $\lbrace \zeta^{\tt{DL}}_{\ell,p}  \rbrace_{\substack{\ell = 1 \ldots L\\ p = 1 \ldots P}}$ taking the form of 
\begin{equation}
\label{eq:SR-decomposition}
	\zeta^{\tt{DL}}_{\ell,p} = \log_2(1+\zeta_{\ell}^{\tt{DL}}) - \log_2(1+\zeta_{p,\tt{DFRC}}^{\tt{Eve}} ), \qquad \forall  \ell , p
\end{equation}
and such that $\zeta_{\ell}^{\tt{DL}} > \zeta_{p,\tt{DFRC}}^{\tt{Eve}}$, in addition to $\min\nolimits_{\ell,p} \zeta^{\tt{DL}}_{\ell,p} = \zeta^{\tt{DL}} $. Therefore, we can now impose secrecy-rate constraints for each $\ell^{th}$ \ac{DL} communication user and $p^{th}$ eavesdropper as follows
\begin{equation}
\Big[
\log_2(1+\SINR_{\ell}^{\tt{DL}})
-
\log_2(1+\SINR_{p,\tt{DFRC}}^{\tt{Eve}})
\Big]^+
\geq
 \zeta^{\tt{DL}}_{\ell,p}, \qquad \forall  \ell , p
\end{equation}
 Since each $\zeta^{\tt{DL}}_{\ell,p}$ is positive, then we can remove the $[]^+$ operator to have 
\begin{equation}
\label{eq:SR-bound}
\log_2(1+\SINR_{\ell}^{\tt{DL}})
-
\log_2(1+\SINR_{p,\tt{DFRC}}^{\tt{Eve}})
\geq
 \zeta^{\tt{DL}}_{\ell,p}, \qquad \forall  \ell , p
\end{equation}
Using \eqref{eq:SR-decomposition} in \eqref{eq:SR-bound}, it suffices to bound 
\begin{equation}
	\SINR_{\ell}^{\tt{DL}} \geq \zeta_{\ell}^{\tt{DL}}, \qquad \forall \ell
\end{equation}
which is the first constraint in appearing in problem $(\mathcal{P}_{1.1})$ within equation \eqref{eq:problem1_1} of the revised manuscript and 
\begin{equation}
	\SINR_{p,\tt{DFRC}}^{\tt{Eve}} \leq \zeta_{p,\tt{DFRC}}^{\tt{Eve}}, \qquad \forall p
\end{equation}	
which is the third constraint in problem $(\mathcal{P}_{1.1})$ within equation \eqref{eq:problem1_1} of the revised manuscript.
A similar argument can be done to obtain the second and fourth constraints in problem $(\mathcal{P}_{1.1})$ within equation \eqref{eq:problem1_1} of the revised manuscript.
We have also replaced the term $\sum\nolimits_{k=1}^K p_k$ appearing in $(\mathcal{P}_1)$ within equation \eqref{eq:problem1} by $\pmb{1}^T \pmb{p}$ appearing in problem $(\mathcal{P}_{1.1})$ within equation \eqref{eq:problem1_1} of the revised manuscript for vector notation.

==> Response/ISMR-comment.tex <==
The authors would like to thank the reviewer for the comment.
We have now added more explanations on the \ac{ISMR} metric as suggested by the comment. 
We have described why the concentration of power in mainlobes is appealing in target localization and tracking applications. 
In particular, this is desired to improve the localization performance of an eavesdropper in direction $\theta_p$, which is assumed to be known.
We have also clarified how the inaccurate location of the eavesdropping targets can be configured by the \ac{ISMR} metric.
In addition, we have clarified that decreasing sidelobe power in certain directions can contribute in attenuating signal-dependent interference and clutter.
Furthermore, we have cited some references (which are \cite{10130609}, \cite{8756034}, and \cite{10018908}) that use the \ac{ISMR} in their design. For example, \cite{10130609} has adopted \ac{ISMR} when designing waveforms for \ac{DFRC} for hybrid linear-nonlinear precoding.
We have also cited a patent \cite{wasiewicz2015method} relating to a useful application for ground-based radars, which utilizes the concept of \ac{ISMR} indirectly, where the beamformers are designed to amplify the receiving mainlobe and null the sidelobe pointing in the direction of the clutter.



==> Response/R2C6.tex <==
The authors would like to thank the reviewer for the comment.
After repeating the entire simulations due to the many changes while addressing the comments, we have now reduced the number of numerical points in simulations where the curves look confusing. 
This includes the following figures in the updated manuscript: 
Fig. \ref{fig:pow_consumption_1}, 
Fig. \ref{fig:pow_consumption_2}, 
Fig. \ref{fig:DL_secrecy_1},
Fig. \ref{fig:DL_secrecy_2},
Fig. \ref{fig:DL_secrecy_3}, and
Fig. \ref{fig:UL_secrecy_1}.


==> Response/R2C7.tex <==
The authors would like to thank the reviewer for the comment.
We have now included the units of all parameters.
First we have replaced all occurrences of $\sigma_n$, $\sigma_p$, $\sigma_\ell$ by $\sigma_n^2$, $\sigma_p^2$, $\sigma_\ell^2$ and used $\dBm$ as unit \cite{8207426}.
For $\zeta^{\tt{UL}}$ and $\zeta^{\tt{DL}}$, we have kept them on a linear scale and they are unit-less, as they represent bounds on the \ac{SINR}, which is a ratio of powers, hence unit-less.

==> Response/R3-C2-response.tex <==
The authors would like to thank the reviewer for the comment.
The eavesdropper \acp{AoA} are assumed to be known in this paper, and can be estimated through a previous stage.
The knowledge of \ac{AoA} imposes partial knowledge about the eavesdroppers absolute position. Motivated by this, the \ac{DFRC} \ac{BS} optimizes its transmit waveform in order to process its received signal for estimating other sensing parameters such us delay and/or Doppler, as well as tracking.
In optimizing the \ac{ISMR} towards the known eavesdropper \acp{AoA}, the radar \ac{SNR} is optimized as a consequence, therefore any distance estimation algorithm integrated at the \ac{DFRC} \ac{BS} is expected to perform better, thereby improving the localization performance of the eavesdroppers \cite{9724174}.
Many other \ac{ISAC} works assume knowledge of target \acp{AoA} in order to enhance either detection or localization performance. Herein we name a few:
The work in \cite{9724174} optimizes signal-clutter-noise ratio under known target \ac{AoA}. 
Moreover, the work in \cite{9916163} considers knowledge of target \acp{AoA} while optimizing the transmit beampattern gain.
In addition, the work in \cite{9537599} design a finite impulse response filter optimized given the \ac{AoA} of the target in order to optimize the radar \ac{SINR}.
Furthermore, the work in \cite{10254508} considers transmit beamforming towards known angles.
Other works that assume knowledge of target \acp{AoA} include \cite{9909807}, \cite{demirhan2023cell}, \cite{10054402}.

==> Response/R3C6.tex <==
The authors would like to thank the reviewer for the comment.
Indeed, a practical setup should be considered to show performance in order to make a wide applicability.
For this, we have repeated our entire simulations by considering a typical communication setup. 
We have included both small-scale and large-scale fading, taking into account shadowing and fading, as well as different channel distributions such as Rician and Rayleigh distributions, and analyzed the performance accordingly. 
we have also set the positions of different nodes within the cell radius and studied the performance according to their positions. 
We have also studied how these positions can impact the resulting secrecy rate performance. 

==> Response/R4-C2-response.tex <==
The authors would like to thank the reviewer for the comment.
The eavesdropper \acp{AoA} are assumed to be known in this paper, and can be estimated through a previous stage.
The knowledge of \ac{AoA} imposes partial knowledge about the eavesdroppers absolute position. Motivated by this, the \ac{DFRC} \ac{BS} optimizes its transmit waveform in order to process its received signal for estimating other sensing parameters such us delay and/or Doppler, as well as tracking.
In optimizing the \ac{ISMR} towards the known eavesdropper \acp{AoA}, the radar \ac{SNR} is optimized as a consequence, therefore any distance estimation algorithm integrated at the \ac{DFRC} \ac{BS} is expected to perform better, thereby improving the localization performance of the eavesdroppers \cite{9724174}.
Many other \ac{ISAC} works assume knowledge of target \acp{AoA} in order to enhance either detection or localization performance. Herein we name a few:
The work in \cite{9724174} optimizes signal-clutter-noise ratio under known target \ac{AoA}. 
Moreover, the work in \cite{9916163} considers knowledge of target \acp{AoA} while optimizing the transmit beampattern gain.
In addition, the work in \cite{9537599} design a finite impulse response filter optimized given the \ac{AoA} of the target in order to optimize the radar \ac{SINR}.
Furthermore, the work in \cite{10254508} considers transmit beamforming towards known angles.
Other works that assume knowledge of target \acp{AoA} include \cite{9909807}, \cite{demirhan2023cell}, \cite{10054402}.

==> Response/R4C3.tex <==
The authors would like to thank the reviewer for the comment.
As we have now changed the entire simulation parameters to follow a typical \ac{mmWave} communication setup by picking the numerology followed in \cite{8207426}, we have adjusted our noise power levels accordingly. 
In particular, we now use the following equation relating the thermal noise power, usually the dominating noise power in a receiver's frontend, to several system parameters
\begin{equation}
	\sigma^2 
	=
	N_F \times K_B \times T_0 \times B
\end{equation}
where 
$N_F$ is the noise figure at the receiving node,
$K_B$ is Boltzmann's constant, which is $1.38 \times 10^{-23}$,
$T_0$ is the reference receiver temperature which is $290$ degrees Kelvin, and
$B$ is the operator bandwidth.
Following \cite{8207426}, it has been mentioned that thermal noise \ac{PSD} is typically $-174 \dBmpHz$, which can be obtained from the above equation by setting the bandwidth $B = 1 \Hz$ and the noise figure $N_F = 0 \dB$. Hence
\begin{equation}
	1 \times (1.38 \times 10^{-23}) \times 290 \times 1
	=
	-174 \dBmpHz
\end{equation}
Hence noise power for a device with $N_F = 7\dB$ \cite{8207426} and operating bandwidth of $0.5 \GHz$ is about $-80\dBm$ \cite{8207426}.
On the other hand, since we are now including pathloss and shadowing as part of our simulation flow, $-80\dBm$ for noise power is typically acceptable, as the pathloss between \ac{DFRC} \ac{BS} and \ac{DL} is of the order of $-60\dBm$ with the given parameters, hence an \ac{SNR} of the order of $20\dB$, which is typical \cite{8207426}.
To make a wide range of applicability, as operating bandwidths and noise figures can vary on a device basis, we have spanned a very wide range of noise power levels as, for instance now:
In Fig. \ref{fig:pow_consumption} in the updated manuscript, which corresponds to Fig. \ref{fig:pow_consumption_all} in this response letter, we have picked $\sigma_n^2 = -60\dBm$ and $\sigma_n^2 = -80\dBm$. Furthermore,
in Fig. \ref{fig:DL_secrecy_1} in the updated manuscript, which corresponds to Fig. \ref{fig:DL_secrecy_1_all} in this response letter, we have spanned a range of $-170 \dBm$ up till $-22\dBm$. In addition,
in Fig. \ref{fig:DL_secrecy_2} in the updated manuscript, which corresponds to Fig. \ref{fig:DL_secrecy_2_all} in this response letter, we have also spanned a wide range from $-70 \dBm$ up till $-7\dBm$.


==> Response/R4C4.tex <==
The authors would like to thank the reviewer for the comment.
We have added a simulation to compare the optimized results of the proposed system with and without AN.
We have compared both variants in terms of $(i)$ achievable secrecy rate vs total consumed power and $(ii)$ in terms of the feasibility rate of the problem.
We have observed that not only \ac{AN} is helpful for achieving a given secrecy rate under much less power, but also that \ac{AN} allows a better feasibility of the proposed algorithm.

==> Response/R4C5.tex <==
The authors would like to thank the reviewer for the comment.
% ISO
The isotropic design is a widely used benchmark in different works on physical layer security. For instance,
\cite{8758975} used the isotropic approach as benchmark for \ac{AN} relaying schemes.
\cite{6951465} used isotropic power distribution to see the benefit of equally distributing the power between AN generation and cooperative beamforming.
Another reference that utilize isotropic design as benchmark is \cite{6853867}.
% SRCS
Furthermore,
the SRCS method \cite{9199556} is an optimized competing scheme in a sense that it minimizes the eavesdroppers \ac{SNR} under communications, radar and power budget constraints.
% SCA w/o AN
We have now included the proposed scheme without \ac{AN} as another optimized competing scheme to compare with, as part of the action item of the previous comment, which is also optimized but  without \ac{AN}.
% no AN + Fig 4
The no \ac{AN} \ac{ZF} scheme was designed for communications only with the intention to have an idea when secrecy optimization becomes less important, i.e. when the eavesdroppers become more noisy (large $\sigma_p^2$) as per Fig. \ref{fig:DL_secrecy_2} in the updated manuscript, which corresponds to Fig. \ref{fig:DL_secrecy_2_all} in this response letter.


==> Response/SingleAntenna-response.tex <==
The authors would like to thank the reviewer for the comment.
The uplink and downlink users are indeed single-antenna users and we have taken the necessary action, thanks to this comment, to highlight that both uplink and downlink users are equipped with single antennas.

==> Response/UL-to-DL-interference-and-model.tex <==
%The authors would like to thank the reviewer for the comment.
Yes, we agree with the Reviewer that the $\ell^{th}$ legitimate receiver should include the \ac{UL} signals the same way the $p^{th}$ eavesdropper does. 
We have went through the system model and proposed algorithm to accommodate this \ac{UL}-to-\ac{DL}-interference.  
The modifications are detailed in the \textbf{Action} items below.
For the channel models, we have also taken action and clarified that this difference is due to the scenario considered with a strong \ac{LoS} component between the eavesdropping targets and the \ac{DFRC} \ac{BS}, which is suitable for \acp{UAV} type applications \cite{10098686}, where a dominant air-ground LoS links exist.

==> Response/acronym-package-response.tex <==
The authors would like to thank the reviewer for the comment.
We are now using the {\tt{acronym}} package of {\LaTeX} to ensure that all acronyms are properly abbreviated. 
For this, we have created a file called {\tt{acronyms.tex}} that contains all abbreviations used in the manuscript. 
For self interference, we have added the following line in {\tt{acronyms.tex}}:
\begin{verbatim}
.
.
\acro{SI}{self interference}
.
.
\end{verbatim}
As a result, every occurrence of 'self interference' is replaced by \ac{SI} and the first occurrence of \ac{SI} will be automatically defined.  

==> Response/bolded-statements.tex <==
The authors would like to thank the reviewer for the comment.
We have now bolded \textbf{input}, \textbf{while}, \textbf{for} and other statements in Algorithm 1.

==> Response/clutter-response.tex <==
The authors would like to thank the reviewer for the comment.
We agree with the reviewer that the model does not specifically separate the communication and sensing signals, and so both are part of the same signal, which is one of the main motivations of ISAC.
Indeed, the clutter has an impact on both downlink and uplink transmissions and is taken into account as part of the downlink and uplink communication channels.
We have taken the necessary action and clarified during the introduction of both channels that indeed the clutter is part of the Rayleigh fading channels and therefore it will impact uplink transmissions and downlink  receptions.


==> Response/constraint38-response.tex <==
The authors would like to thank the reviewer for bringing this typo to our attention.
Indeed, the $ p_k^{(m)}$ should be $p_k$.
The corrected constraint is now 
\begin{equation}
\begin{split}
	2 p_k \pmb{h}^H_{t,k}
	[\pmb{\Phi}_k^{(m)}]^{-1}
	 \pmb{h}_{t,k}
	 & \geq 
	  \zeta_{k}^{\tt{UL}}
	 +
	  p_k
	  \pmb{h}^H_{t,k}
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{\Phi}_k
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{h}_{t,k}.
\end{split}
\end{equation}
Then by dividing by $p_k$ on all sides, we can re-write the constraint as 
\begin{equation}
	\underbrace{\frac{\zeta_{k}^{\tt{UL}}}{p_k}
	  +
	  \pmb{h}^H_{t,k}
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{\Phi}_k
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{h}_{t,k}
	-
	2  \pmb{h}^H_{t,k}
	[\pmb{\Phi}_k^{(m)}]^{-1}
	 \pmb{h}_{t,k}}_{\pmb{\Lambda}_k}
	 \leq 0.
\end{equation}
Regarding convexity, the above constraint is now convex in $\pmb{p}, \pmb{V}_1 \ldots \pmb{V}_\ell$ and $\pmb{W}$. 
To show this, we have resorted to second-order condition arguments of  twice differentiable functions.
We have first derived the first-order derivatives of $\pmb{\Lambda}_k$, which are given as follows
\begin{align}
	\frac{\partial \pmb{\Lambda}_k}{\partial p_k}
	&=
	-
	\frac{\zeta_{k}^{\tt{UL}}}{p_k^2},\\
	\frac{\partial \pmb{\Lambda}_k}{\partial p_{k'}}
	&=
	\pmb{h}^H_{t,k}
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{h}_{t,k'}\pmb{h}_{t,k'}^H
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{h}_{t,k}, \quad \forall k' \neq k, \\
	\frac{\partial \pmb{\Lambda}_k}{\partial \pmb{V}_\ell}	% eq (70) in cookbook
	&=
	\frac{\partial \pmb{\Lambda}_k}{\partial \pmb{W}}
	=
	\pmb{C}^H
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{h}_{t,k}
	\pmb{h}_{t,k}^H
	[\pmb{\Phi}_k^{(m)}]^{-1}
	\pmb{C}, \quad \forall \ell.
\end{align}
From the above expressions, we can also derive the Hessian of $\pmb{\Lambda}_k$ which is all-zeros except for its $k^{th}$ diagonal element, which is given by 
\begin{equation}
	\frac{\partial^2 \pmb{\Lambda}_k}{\partial p_k^2}
	=
	\frac{2\zeta_{k}^{\tt{UL}}}{p_k^3}.
\end{equation}
Therefore, the Hessian is a positive semi-definite matrix if and only if $\frac{\partial^2 \pmb{\Lambda}_k}{\partial p_k^2} \geq 0$, which occurs when both $p_k > 0$ and $\zeta_{k}^{\tt{UL}} \geq 0 $.
Note that $\zeta_{k}^{\tt{UL}}$ is a given positive quantity and $p_k$ is already positive due to the feasible set defined by the problem (i.e. element-wise positivity constraint on power vectors $\pmb{p}$).
We conclude that the Hessian is a positive semi-definite matrix, hence the constraint is convex.

==> Response/figures-all-simulations.tex <==
\begin{figure*}[t]
\centering
\subfloat[\textcolor{blue}{$\sigma_n^2 = -80\dBm$}]{\includegraphics[width=2in]{./figuresTexv2/fig2aTex}%
\label{fig:pow_consumption_1_all}}
\hfil
\subfloat[\textcolor{blue}{$\sigma_n^2 = -60\dBm$}]{\includegraphics[width=2in]{./figuresTexv2/fig2bTex}%
\label{fig:pow_consumption_2_all}}
\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig2a_captions.tex}}}
\label{fig:pow_consumption_all}
\end{figure*}


\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig3Tex}
\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig3_captions.tex}}}
	\label{fig:DL_secrecy_1_all}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig4Tex}
\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig4_captions.tex}}}
	\label{fig:DL_secrecy_2_all}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig5Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig5_captions.tex}}}
	\label{fig:DL_secrecy_3_all}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig6Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig6_caption.tex}}}
		\label{fig:UL_secrecy_1_all}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig7Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig7_caption.tex}}}
	\label{fig:bp_1_all}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig8Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig8_captions.tex}}}
	\label{fig:tradeoff_all}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig9Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig9_captions.tex}}}
	\label{fig:tradeoff2_all}
\end{figure}

==> Response/figures-tikz-simulations.tex <==
\begin{figure*}
\centering
\subfloat[\textcolor{blue}{$\sigma_n^2 = -80\dBm$}]{\includegraphics[width=2in]{./figuresTexv2/fig2aTex}%
\label{fig:pow_consumption_1_tikz}}
\hfil
\subfloat[\textcolor{blue}{$\sigma_n^2 = -60\dBm$}]{\includegraphics[width=2in]{./figuresTexv2/fig2bTex}%
\label{fig:pow_consumption_2_tikz}}
\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig2a_captions.tex}}}
\label{fig:pow_consumption_tikz}
\end{figure*}


\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig3Tex}
\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig3_captions.tex}}}
	\label{fig:DL_secrecy_1_tikz}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig4Tex}
\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig4_captions.tex}}}
	\label{fig:DL_secrecy_2_tikz}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig5Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig5_captions.tex}}}
	\label{fig:DL_secrecy_3_tikz}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig6Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig6_caption.tex}}}
		\label{fig:UL_secrecy_1_tikz}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig7Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig7_caption.tex}}}
	\label{fig:bp_1_tikz}
\end{figure}


\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig8Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig8_captions.tex}}}
	\label{fig:tradeoff_tikz}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig9Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig9_captions.tex}}}
	\label{fig:tradeoff2_tikz}
\end{figure}

==> Response/figures-with-channel-conditions.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig3Tex}
\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig3_captions.tex}}}
	\label{fig:DL_secrecy_1_channel}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig4Tex}
\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig4_captions.tex}}}
	\label{fig:DL_secrecy_2_channel}
		\vspace{-0.5cm}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{./figuresTexv2/fig6Tex}
	\caption{\textcolor{blue}{\protect\input{Actions/Captions/Fig6_caption.tex}}}
		\label{fig:UL_secrecy_1_channel}
\end{figure}

==> Response/imperfect-csi-response.tex <==
The authors would like to thank the reviewer for the comment.
We agree that the implicit presence of perfect \ac{CSI} knowledge at the nodes is very ideal, especially for \ac{ISAC}.
We have therefore taken the appropriate action to not only model the imperfect \ac{CSI} case at all nodes, but also to tailor a \ac{BCCD} type method to solve the non-convex problem arising at hand.
In this response comment, and due to space limitations in the updated manuscript, we detail some steps at how we arrive at the imperfect \ac{CSI} problem in equation \eqref{d1:eq:problem1_1_imperfect_csi} of the updated manuscript.
%% Constraint 1
The first constraint in problem \eqref{d1:eq:problem1} of the updated manuscript is given as 
\begin{equation}
\label{eq:constraint-1-w-csi}
	\SINR_{\ell}^{\tt{DL}}
	= 
	\frac{ \pmb{h}_{r,\ell}^H\pmb{V}_\ell\pmb{h}_{r,\ell} } 
	     {\sum\limits_{\substack{k = 1  }}^K p_k \vert q_{k,\ell} \vert^2 + \sum\limits_{\substack{\ell^{'} = 1\\ \ell^{'} \neq \ell}}^L \pmb{h}_{r,\ell}^H\pmb{V}_{\ell^{'}}\pmb{h}_{r,\ell} + \pmb{h}_{r,\ell}^H\pmb{W}\pmb{h}_{r,\ell}  +\sigma_{\ell}^2} \geq \zeta_{\ell}^{\tt{DL}}
\end{equation}
where in the presence of imperfect \ac{CSI} we have that
\begin{equation}
	\pmb{h}_{r,\ell}
	=
	\widehat{\pmb{h}}_{r,\ell}
	+ 
	\Delta \pmb{h}_{r,\ell}, \quad \forall \ell = 1 \ldots L,
\end{equation}
and $\Delta \pmb{h}_{r,\ell}$ is the error on the $\ell^{th}$ \ac{DL} channel satisfying the ellipsoidal uncertainty model, namely \cite{6026260}, \cite{5164911}
\begin{equation}
\Vert 
\pmb{E}_{r,\ell}^{\frac{1}{2}} 
\Delta \pmb{h}_{r,\ell} 
\Vert 
\leq
1, \quad \forall \ell = 1 \ldots L,
\end{equation}
After applying the $\mathcal{S}$-lemma (also known as $\mathcal{S}$-procedure) on the above constraint in equation \eqref{eq:constraint-1-w-csi} herein, we can express the above as a convex semi-definite constraint as follows
\begin{equation}
	\begin{bmatrix}
		\widehat{\pmb{h}}_{r,\ell}^H 
		\pmb{Q}_\ell 
		\widehat{\pmb{h}}_{r,\ell}
		-
		\zeta_{\ell}^{\tt{DL}}
		\sigma_{\ell}^2
		-\zeta_{\ell}^{\tt{DL}}\sum\limits_{\substack{k = 1  }}^K p_k \vert q_{k,\ell} \vert^2 
		-
		s_\ell &
		\widehat{\pmb{h}}_{r,\ell}^H 
		\pmb{Q}_\ell  \\
\pmb{Q}_\ell 
		\widehat{\pmb{h}}_{r,\ell} &
		\pmb{Q}_\ell  + s_\ell \pmb{E}_{r,\ell} 	
	\end{bmatrix}
	\succeq \pmb{0},
	\quad
	s_\ell \geq 0 
\end{equation}
where $\pmb{Q}_\ell = \pmb{V}_\ell - \zeta_{\ell}^{\tt{DL}} \pmb{W} - \zeta_{\ell}^{\tt{DL}} \sum\nolimits_{\ell' \neq \ell} \pmb{V}_{\ell'}$.
This constraint corresponds to constraint \eqref{d1:eq:imperfect-csi-constraint-1} in the updated manuscript. 
%% Constraint 2
For the second constraint arising in the original problem \eqref{d1:eq:problem1} of the updated manuscript, we have that 
\begin{equation}
\label{eq:constraint-2-w-csi}
	\SINR_{k}^{\tt{UL}}
	=
	\frac
	{ p_k\pmb{u}_k^H \pmb{h}_{t,k}\pmb{h}^H_{t,k} \pmb{u}_k }
	{\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K p_{k'} \pmb{u}_k^H \pmb{h}_{t,k'}\pmb{h}^H_{t,k'} \pmb{u}_k  +
	\pmb{u}_k^H \pmb{C}\pmb{Q}\pmb{C}^H \pmb{u}_k + 
	\pmb{u}_k^H \pmb{R}_c \pmb{u}_k +
	\sigma_n^2 \pmb{u}_k^H\pmb{u}_k} 
	\geq  \zeta^{\tt{UL}}_k
\end{equation}
where in the presence of imperfect-\ac{CSI} we have that 
\begin{equation}
	\pmb{h}_{t,k}
	=
	\widehat{\pmb{h}}_{t,k}
	+ 
	\Delta \pmb{h}_{t,k}, \quad \forall k = 1 \ldots K,
\end{equation}
and $\Delta \pmb{h}_{t,k}$ is the error on the $k^{th}$ \ac{UL} channel satisfying the ellipsoidal uncertainty model, namely \cite{6026260}, \cite{5164911}.
\begin{equation}
	\Vert \pmb{E}_{t,k}^{\frac{1}{2}} \Delta \pmb{h}_{t,k} \Vert \leq 1, \quad \forall k.
\end{equation}
We can re-write the constraint in \eqref{eq:constraint-2-w-csi} herein as 
 \begin{equation}
	p_k\pmb{u}_k^H \pmb{h}_{t,k}\pmb{h}^H_{t,k} \pmb{u}_k
	-
	\zeta^{\tt{UL}}
	\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K p_{k'} \pmb{u}_k^H \pmb{h}_{t,k'}\pmb{h}^H_{t,k'} \pmb{u}_k
	\geq  
	\zeta^{\tt{UL}}_k
		\Big( 
	\pmb{u}_k^H \pmb{C}\pmb{Q}\pmb{C}^H \pmb{u}_k + 
	\pmb{u}_k^H \pmb{R}_c \pmb{u}_k +
	\sigma_n^2 \pmb{u}_k^H\pmb{u}_k\Big)
\end{equation}
Now we find a deterministic lower-bound of the upper-bound in the above inequality by utilizing the following bounds in \cite{6026260}
	\begin{equation}
		p_k\pmb{u}_k^H \pmb{h}_{t,k}\pmb{h}^H_{t,k} \pmb{u}_k
		=
		p_k 
		\Vert
		(\widehat{\pmb{h}}_{t,k}
	+ 
	\Delta \pmb{h}_{t,k})^H \pmb{u}_k
		\Vert^2  
		\geq
		p_k
		\Big[ \max (		\Vert
		(\widehat{\pmb{h}}_{t,k})^H \pmb{u}_k
		\Vert -  \Vert\pmb{E}_{t,k}^{-\frac{1}{2}} \pmb{u}_k\Vert
		,0 )
		\Big]^2
	\end{equation}
	
	\begin{equation}
		p_{k'} \pmb{u}_k^H \pmb{h}_{t,k'}\pmb{h}^H_{t,k'} \pmb{u}_k
  =
  p_{k'} 
  \Vert
		(\widehat{\pmb{h}}_{t,k'}
	+ 
	\Delta \pmb{h}_{t,k'})^H \pmb{u}_k
		\Vert^2
		\leq 
		p_{k'}
		\Big[
		\Vert
		\widehat{\pmb{h}}_{t,k'}^H \pmb{u}_k
		\Vert 
		+
		\Vert \pmb{E}_{t,k'}^{-\frac{1}{2}} \pmb{u}_k\Vert
		 \Big]^2
	\end{equation}
Combining the above two constraints, we have that
	\begin{equation}
		p_k 
		(		\Vert
		\widehat{\pmb{h}}_{t,k}^H \pmb{u}_k
		\Vert - \Vert \pmb{E}_{t,k}^{-\frac{1}{2}} \pmb{u}_k\Vert)^2
		-
		\zeta^{\tt{UL}}_k
	\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K
		p_{k'}
		(				\Vert
		\widehat{\pmb{h}}_{t,k'}^H \pmb{u}_k
		\Vert 
		+
		 \Vert \pmb{E}_{t,k'}^{-\frac{1}{2}} \pmb{u}_k\Vert )^2
		\geq 
		\zeta^{\tt{UL}}_k
		\Big( 
	\pmb{u}_k^H \pmb{C}\pmb{Q}\pmb{C}^H \pmb{u}_k + 
	\pmb{u}_k^H \pmb{R}_c \pmb{u}_k +
	\sigma_n^2 \pmb{u}_k^H\pmb{u}_k\Big)
\end{equation}
This constraint corresponds to constraint \eqref{d1:eq:imperfect-csi-constraint-2} in the updated manuscript, which has been re-written in a much more compact form.
%% Constraint 3
The third constraint in the original problem \eqref{d1:eq:problem1} of the updated manuscript is
\begin{equation}
\label{eq:constraint-3-w-csi}
	\SINR_{p,\tt{DFRC}}^{\tt{Eve}}
	=
	\frac
	{\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)}
	{\sum\limits_{\substack{k = 1  }}^K p_k \vert g_{k,p} \vert^2 + 
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2 }
	 \leq  \zeta_{p,\tt{DFRC}}^{\tt{Eve}}
\end{equation}
where in the presence of imperfect-\ac{CSI} we have that 
\begin{equation}
\label{eq:uncertain-gkp}
	g_{k,p}
	=
	\widehat{g}_{k,p}
	+ 
	\Delta g_{k,p}, \quad \forall k = 1 \ldots K, \quad \forall p = 1 \ldots P
\end{equation}
and we assume that 
\begin{equation}
	\Vert \Delta g_{k,p} \Vert \leq \epsilon_{k,p}, \quad \forall k,p.	
\end{equation}
We can re-write the above constraint in equation \eqref{eq:constraint-3-w-csi} herein as 
\begin{equation}
\label{constraint-3-rewritten}
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)
	-
	\zeta_{p,\tt{DFRC}}^{\tt{Eve}}
	\sum\limits_{\substack{k = 1  }}^K p_k \vert g_{k,p} \vert^2 
	\leq
	\zeta_{p,\tt{DFRC}}^{\tt{Eve}}
	\Big(
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2
	\Big)
\end{equation}
where we can bound the \ac{CSI} as 
	\begin{equation}
		p_{k} \vert g_{k,p} \vert^2
		=
		p_{k} \vert  \widehat{g}_{k,p} +  \Delta g_{k,p} \vert^2
		\geq 
		p_{k} 
		\Big[
		\vert \widehat{g}_{k,p} \vert - \epsilon_{k,p}
		\Big]^2
	\end{equation}	
Hence utilizing the above bound as an upper bound on the lower bound in \eqref{constraint-3-rewritten}, we have
\begin{equation}
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)
	-
	\zeta_{p,\tt{DFRC}}^{\tt{Eve}}
	\sum\limits_{\substack{k = 1  }}^K p_k 
	(		\vert \widehat{g}_{k,p} \vert
	-
	 \epsilon_{k,p} )^2
	\leq
	\zeta_{p,\tt{DFRC}}^{\tt{Eve}}
	\Big(
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2
	\Big)
\end{equation}
This constraint corresponds to constraint \eqref{d1:eq:imperfect-csi-constraint-3} in the updated manuscript, which has been re-written in a much more compact form.
%% Constraint 4
The fourth constraint in the original problem \eqref{d1:eq:problem1} of the updated manuscript is
	\begin{equation}
	\label{eq:constraint-4-w-csi}
	\SINR_{p,k}^{\tt{Eve}}
	=
	\frac
	{ p_k \vert g_{k,p} \vert^2  }
	{\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K p_{k'} \vert g_{k',p} \vert^2 + \vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{Q}\pmb{a}_{N_T}(\theta_p) + \sigma_p^2}
	\leq \zeta_{p,k}^{\tt{Eve}}
	\end{equation}
	where $g_{k,p}$ follows equation \eqref{eq:uncertain-gkp} herein. We can re-write \eqref{eq:constraint-4-w-csi} herein as 
	\begin{equation}
	 p_k \vert g_{k,p} \vert^2 
	 -
	 \zeta_{p,k}^{\tt{Eve}}\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K p_{k'} \vert g_{k',p} \vert^2
	 \leq 
	 \zeta_{p,k}^{\tt{Eve}} 
	 \big(\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{Q}\pmb{a}_{N_T}(\theta_p) + \sigma_p^2
	 \big)
	\end{equation}
	Next, we aim at upper bounding the lower bound via a deterministic bound using the following
\begin{equation}
		p_k \vert g_{k,p} \vert^2 
		=
		p_k \vert \widehat{g}_{k,p}
	+ 
	\Delta g_{k,p}\vert^2 
	\leq
	p_k 
	\Big[
	\vert \widehat{g}_{k,p} \vert
	+
	\epsilon_{k,p}
	\Big]^2
	\end{equation}
	
	\begin{equation}
		p_{k'} \vert g_{k',p} \vert^2
		=
		p_{k'} \vert  \widehat{g}_{k',p} +  \Delta g_{k',p} \vert^2
		\geq 
		p_{k'} 
		\Big[
		\vert \widehat{g}_{k',p} \vert - \epsilon_{k',p}
		\Big]^2
	\end{equation}
Hence, with the aid of the above, we can say that \eqref{eq:constraint-4-w-csi} corresponds to 
	\begin{equation}
	 p_k
	 (\vert \widehat{g}_{k,p} \vert
	+
	\epsilon_{k,p} )^2
	 -
	 \zeta_{p,k}^{\tt{Eve}}\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K p_{k'} (		\vert \widehat{g}_{k',p} \vert
	-
	\epsilon_{k',p} )^2
	 \leq 
 \zeta_{p,k}^{\tt{Eve}} 
	 \big(\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{Q}\pmb{a}_{N_T}(\theta_p) + \sigma_p^2
	 \big)
	\end{equation}
This constraint corresponds to constraint \eqref{d1:eq:imperfect-csi-constraint-4} in the updated manuscript, which has been re-written in a much more compact form.
After formulating the new \ac{FD} \ac{ISAC} power minimization with imperfect-\ac{CSI} optimization problem in \eqref{d1:eq:problem1_1_imperfect_csi} of the updated manuscript, we further devise a \ac{BCCD} type method that aims at solving the non-convex problem at hand.
This method is detailed in Section \ref{d1:sec:imperfect-csi} of the updated manuscript just after introducing the new \ac{FD} \ac{ISAC} power minimization with imperfect-\ac{CSI} optimization problem in equation  \eqref{d1:eq:problem1_1_imperfect_csi}.















==> Response/learning-response.tex <==
The authors would like to thank the reviewer for the comment and for drawing our attention onto the insightful survey, which we now cite in this manuscript.
% security issues 
We have now identified additional security issues, as well as vulnerabilities, in future wireless communications, over \ac{B5G} wireless networks and \ac{IoT}, such as limited processing power, memory capacity, battery life, and network bandwidth, in addition to threats, impersonation attacks and routing attacks. 
% DL
In addition, we have highlighted how \ac{DL}-based techniques can turn out to be effective for future wireless communications, but at the same time, can suffer from high complexity if not designed properly. 
% EL
We have also discussed how \ac{EL} can be used to distribute the implementation of \ac{DL} methods over multiple edge devices, thereby reducing computational complexity and malicious attacks.
% as far as we are concerned
Finally, we have mentioned a possible research direction related to the \ac{SCA}-based method for \ac{FD} \ac{ISAC} system, which may exhibit a relatively large number of iterations. In particular, the \ac{EL} philosophy can be adopted to distribute the computations of the proposed \ac{SCA} optimization method, thereby reducing computational complexity.

==> Response/proof-rank-1-response.tex <==
The authors would like to thank the reviewer for the comment.
We have revised the proof and have done necessary amendments and modifications. For example, thanks to comment 03 where the constraint in equation \eqref{eq:constraint38} of the updated manuscript had to be corrected then put in a convex form, there is a missing term that had to be added to equation \eqref{eq:dual-formulation} of the revised manuscript.
Then, $\pmb{\Gamma}$ has been amended to contain an additional positive semi-definite term in equation \eqref{eq:ammended-gamma-expression} of the updated manuscript.
Also, there was a missing statement in the first version that has now been modified. 
In general, the rank-one optimality is still preserved due to the convexity of problem $(\mathcal{P}_{1.3}^{(m)})$.

==> Response/related-work-response.tex <==
The authors would like to thank the reviewer for the comment and for bringing this work to our attention. 
The mentioned papers were published after the submission of this manuscript. We have now added them to the reference list.
%Regarding the potential security concerns that arise due to \ac{FD} \ac{ISAC} systems.
%Wireless communications have an inherent broadcast nature, so security is a major issue. With the introduction of \ac{ISAC}, this issue will aggravate even further.
%Integrating sensing capabilities over communication networks exposes previously unknown vulnerabilities and security problems to unauthorized sensing that must be addressed.
%Specifically, \ac{ISAC} signals are intended to carry both sensing and transmission information. In \ac{FD} \ac{ISAC} systems, these issues can aggravate more as more signals are being exchanged. 
%As a result, while sensing targets, the \ac{ISAC} signal utilized for sensing would hit the target with a significant amount of power, where that particular signal also contains communication information, unlike a pure chirp or radar-only signal. 
%Motivated by this security concern, we push the limits of \ac{FD} \ac{ISAC} systems a step further enabling \ac{FD} \ac{ISAC} to operate in a secure way.
We have then emphasized on the new technical challenge introduced in secure \ac{FD} \ac{ISAC} systems. 
In particular, we don't want to simply design ISAC beamformers to perform sensing and communication tasks, but we also want these beamformers to be able to achieve good secrecy rates via \ac{AN} generation and to guarantee a certain ISMR level to enhance further localization performance. 
\textit{In other words, we reveal minimal communication information towards the mainlobes specified by \ac{ISMR}, thanks to the \ac{DL} secrecy rate consideration within the formulation of our optimization problem. This allows us to further localize malicious targets without exposing the communication information integrated in the \ac{ISAC} signal. In addition, we also want the \ac{UL} secrecy to be good as well.}
The new technical challenge is to design the \ac{ISAC} beamformers and the \ac{ISAC} \ac{AN} statistics so as to achieve the three main functionalities in \ac{FD} \ac{ISAC}, namely sensing, communication and secrecy performance, simultaneously, within the same \ac{ISAC} signal.
% paper 1
%Next, we have also elaborated and compared our work to the existing works mentioned in this comments, i.e. \cite{10158711} and \cite{10159012} (within the references of this response letter).
The authors in \cite{10158711} address the \ac{FD} in an \ac{ISAC} communication setting, from power optimization and beamforming perspectives, however, there are differences that we have highlighted, such as the choice of the radar metric, i.e. the \ac{ISMR} to enhance the sensing performance for localizing the malicious targets. In doing so, our model regards the target localization part of the \ac{ISAC} signal from a security perspective.
Furthermore, we have also leveraged \ac{AN} matrix optimization, which will further aid in obfuscating the communication information towards those malicious users, through \ac{AN} generation. 
Therefore, our problem essentially differs in how the total power is being invested onto the \ac{FD} \ac{ISAC} system and how the \ac{AN} covariance and beamforming vectors distribute minimal power in order to guarantee given \ac{UL}/\ac{DL} secrecy rates at a given \ac{ISMR} level.
% paper 2
Furthermore, the work in \cite{10159012} focuses primarily on an \ac{FD} \ac{ISAC} setup to represent the "echo-miss" problem, which is a scenario emerging from high residual \ac{SI} that can mask the radar echo, thereby missing the received echo due to target presence. To address this, the authors of \cite{10159012} proposed formulating an optimization problem to fulfill \ac{UL}/\ac{DL} communication data rates and generate transmit, receive, and post-\ac{SI} beamformers. 
When comparing to  \cite{10159012}, there are also some notable differences. 
First, the sensing measure used in \cite{10159012} is the radar beampattern power output for only a single target, without taking into account clutter components.
Also, we model potential communication leaks onto multiple radar targets, which then enables us to define key security metrics such as \ac{UL} and \ac{DL} secrecy rates in the proposed secure \ac{FD} \ac{ISAC} scheme.


==> Response/thetap-are-known-or-not.tex <==
The authors would like to thank the reviewer for the comment.
The angles $\theta_p$ are not known to the \ac{DFRC} \ac{BS}, and the problem we are faced in can be translated to a detection-type problem, instead of an estimation one.
This is interesting in applications such as beamscanning, where the \ac{DFRC} \ac{BS} performs secure \ac{FD} communications, but at the same time intends to create beams in certain directions around $\theta_p$ to detect presence of malicious eavesdropping targets, but in a secure way.
An illustration of the beamscan while probing for the $p^{th}$ eavesdropping target is given in Fig. \ref{fig:beamscan}, where the \ac{DFRC} \ac{BS} tests in directions for the presence/absence of a target via hypothesis testing on the received \ac{UL} signal described in equation \eqref{d1:eq:BS-signal} of the revised manuscript.
We have depicted the case of a single target for clarity.
For multiple targets, we can extend this notion to a multitarget detection problem, via M-ary hypothesis testing problem \cite{7849236}.
For this purpose, the \ac{DFRC} \ac{BS} can create multiple beams for target sensing without knowing the target locations, then scan them simultaneously and test via M-ary hypothesis testing \cite{7849236}. 
The \ac{DFRC} \ac{BS} listens to this back-scattered echo from the presence of eavesdropping targets in scanning directions $\theta_p$ in equation \eqref{d1:eq:BS-signal} of the updated manuscript and can use this signal $\pmb{y}^{\tt{DFRC}}$ to test for presence/absence of eavesdroppers in those scanning directions $\theta_p$.
If an eavesdropping target is present, we can further infer extra sensing information of that target, e.g. its \ac{RCS} to infer how big the eavesdropper is, doppler to compute its speed if it is moving, and delay from the \ac{DFRC} \ac{BS} to calculate the distance relative to the \ac{DFRC} \ac{BS}.
Note that thanks to the proposed secure \ac{FD} \ac{ISAC}, the \ac{DFRC} \ac{BS} can securely perform its detection tasks, without exposing the communication information within the \ac{ISAC} waveform \pmb{x} given in equation \eqref{d1:eq:Tx-signal-BS} of the revised manuscript, thanks to the secrecy constraints introduced in our optimization framework.
Therefore, the \ac{DFRC} \ac{BS} can test for simulateneous target presence, while covering the information signals, which would guarantee a high secrecy rate. 
In this article, we focus on the beam design aspect, through the ISMR constraint of the secure FD ISAC optimization problem, to help with the detection procedure carrier out at a later stage at the \ac{DFRC} \ac{BS} upon receiving $\pmb{y}^{\tt{DFRC}}$.
We are sorry for the confusion and we have added some context to make it more clear.

%We have in mind an application that we illustrate in this response in Fig. \ref{fig:beamscan}, i.e. a beamscanning application. 
%When the beam is steered towards an angle where the target of interest is found, then by maximizing the output power of the Bartlett beamformer, $P(\theta_0)$, then we are also maximizing the probability of detection of a source in that direction. Even more, this boost in Bartlett beamforming power also improves performance localization algorithms aiming at utilizing information embedded in the reflection coefficient, such as distance (range) and time of arrival. 
%The optimization is done only on the beamforming matrix $\pmb{W}$ to optimize for the output power of the beamformer and the communication user rates in the presence of imperfect CSI. 
\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{./figures/beamscan.pdf}
	\caption{A beamscan application for the proposed secure \ac{FD} \ac{ISAC} system. Here $\Delta$ defines an angular grid for the beamscan.}
	\label{fig:beamscan}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> sections/imperfect-csi.tex <==
The authors would like to thank the reviewer for the comment.
We have considered a perfect CSI knowledge since it's a common simplifying assumption which is used in several \ac{ISAC} works including \cite{9652071}, \cite{8386661}, \cite{9124713}, \cite{9724174}, \cite{9585492}, \cite{9838548}.
Following the reviewers' comment, we now present an imperfect \ac{CSI} optimization framework tailored for the secure \ac{FD} \ac{ISAC} model at hand. We have also developed a suitable algorithm to solve the resulting optimization problem, in order to show that a solution is possible. 
Please note that the algorithm has not been added in the updated manuscript, due to lack of space, but we have included it here so that we convince the reviewer that imperfect CSI knowledge does not change the main steps of the optimization framework, and the extension to the imperfect knowledge can be a natural extension of our current work.
Therefore, it will be fully included in a followup paper, along with its analysis and insights.
%The implicit presence of perfect \ac{CSI} knowledge at all given nodes in an \ac{ISAC} system may seem to ideal.
%It is worth noting that so far, the proposed \ac{FD} \ac{ISAC} power minimization algorithm is tailored for the perfect \ac{CSI} case, i.e. the \ac{DFRC} \ac{BS} has perfect channel knowledge of $\pmb{h}_{t,k}, \pmb{h}_{r,k}$ and $g_{k,p}$.
%In reality, this knowledge cannot be perfect as inaccurate estimation and quantization errors, as well as outdated channel effects, are part of transmit and receive paths.
In order to model imperfect \ac{CSI}, the \ac{DFRC} \ac{BS} has access to \ac{CSI} information in the form
\begin{align}
	\pmb{h}_{r,\ell}
	&=
	\widehat{\pmb{h}}_{r,\ell}
	+ 
	\Delta \pmb{h}_{r,\ell}, \quad \forall \ell,\\
	\pmb{h}_{t,k}
	&=
	\widehat{\pmb{h}}_{t,k}
	+ 
	\Delta \pmb{h}_{t,k}, \quad \forall k,	\\
	g_{k,p}
	&=
	\widehat{g}_{k,p}
	+ 
	\Delta g_{k,p}, \quad \forall k,p.
\end{align}
Notice that we introduce \ac{CSI} errors integrated within 
$\Delta \pmb{h}_{r,\ell}$ for the $\ell^{th} $ \ac{DL} channel,
$\Delta \pmb{h}_{t,k}$ for the $k^{th}$ \ac{UL} channel, and
$\Delta g_{k,p}$ for the \ac{SISO} channels between the $p^{th}$ eavesdropper and the $k^{th}$ \ac{UL} user. 
For simplicity, the \ac{UL}-to-\ac{DL} interference is herein modeled with perfect \ac{CSI}.
Moreover, the \ac{CSI} available estimates are, therefore, $\widehat{\pmb{h}}_{r,\ell}$, $\widehat{\pmb{h}}_{t,k}$, and $\widehat{g}_{k,p}$.
We now design a robust version of problem \eqref{eq:problem1_1} of the updated manuscript.
Furthermore, we assume the imperfect \ac{CSI} quantities to be deterministic and norm-bounded, i.e. the errors are bounded as follows \cite{6026260}, \cite{5164911}
\begin{align}
\label{DL-pert-set}
\Vert 
\pmb{E}_{r,\ell}^{\frac{1}{2}} 
\Delta \pmb{h}_{r,\ell} 
\Vert 
&\leq
1, \quad \forall \ell, \\
\label{UL-pert-set}
\Vert \pmb{E}_{t,k}^{\frac{1}{2}} \Delta \pmb{h}_{t,k} \Vert &\leq 1, \quad \forall k, \\
\label{eve-pert-set}
\Vert \Delta g_{k,p} \Vert &\leq \epsilon_{k,p}, \quad \forall k,p.	
\end{align}
where $\pmb{E}_{r,\ell}$ and $\pmb{E}_{t,k}$ controls the ellipsoidal shape of the \ac{CSI} perturbation set on the $\ell^{th}$ \ac{DL} channel and $k^{th}$ \ac{UL} channel, respectively. 
Note that we can scale the upper bounds of \eqref{DL-pert-set} and \eqref{UL-pert-set} simply by scaling $\pmb{E}_{r,\ell}$ and $\pmb{E}_{t,k}$.
On the other hand, as we assume a \ac{SISO} link between the $p^{th}$ eavesdropper and the $k^{th}$ \ac{UL} user, we bound the \ac{CSI} error by $\epsilon_{k,p}$.

%% Constraint 1
The first constraint of problem \eqref{eq:problem1_1} of the updated manuscript taking into account \ac{CSI} errors in the \ac{DL} can be re-written via the $\mathcal{S}-$lemma (also known as $\mathcal{S}$-procedure) as 
\begin{equation}
\label{eq:imperfect-csi-constraint-1}
	\begin{bmatrix}
		\widehat{\pmb{h}}_{r,\ell}^H 
		\pmb{Q}_\ell 
		\widehat{\pmb{h}}_{r,\ell}
		-
		\zeta_{\ell}^{\tt{DL}}
		\sigma_{\ell}^2
		-\zeta_{\ell}^{\tt{DL}}\sum\limits_{\substack{k = 1  }}^K p_k \vert q_{k,\ell} \vert^2 
		-
		s_\ell &
		\widehat{\pmb{h}}_{r,\ell}^H 
		\pmb{Q}_\ell  \\
\pmb{Q}_\ell 
		\widehat{\pmb{h}}_{r,\ell} &
		\pmb{Q}_\ell  + s_\ell \pmb{E}_{r,\ell}	
	\end{bmatrix}
	\succeq \pmb{0},
\end{equation}
where $\pmb{Q}_\ell = \pmb{V}_\ell - \zeta_{\ell}^{\tt{DL}} \pmb{W} - \zeta_{\ell}^{\tt{DL}} \sum\nolimits_{\ell' \neq \ell} \pmb{V}_{\ell'}$, $\forall \ell$ and $\exists
	s_\ell \geq 0$.
This means we can treat $s_\ell$ as a slack variable, while considering the positive semi-definite constraint in \eqref{eq:imperfect-csi-constraint-1}.
%% Constraint 2
For the second constraint arising in problem \eqref{eq:problem1_1} of the updated manuscript, we have that 
\begin{equation}
\label{eq:constraint-2-w-csi}
	\SINR_{k}^{\tt{UL}}
	=
	\frac
	{ p_k\pmb{u}_k^H \pmb{h}_{t,k}\pmb{h}^H_{t,k} \pmb{u}_k }
	{\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K p_{k'} \pmb{u}_k^H \pmb{h}_{t,k'}\pmb{h}^H_{t,k'} \pmb{u}_k  +
	\pmb{u}_k^H \pmb{C}\pmb{Q}\pmb{C}^H \pmb{u}_k + 
	\pmb{u}_k^H \pmb{R}_c \pmb{u}_k +
	\sigma_n^2 \pmb{u}_k^H\pmb{u}_k} 
	\geq  \zeta^{\tt{UL}}_k
\end{equation}
where in the presence of imperfect-\ac{CSI} we have that 
\begin{equation}
	\pmb{h}_{t,k}
	=
	\widehat{\pmb{h}}_{t,k}
	+ 
	\Delta \pmb{h}_{t,k}, \quad \forall k = 1 \ldots K,
\end{equation}
and $\Delta \pmb{h}_{t,k}$ is the error on the $k^{th}$ \ac{UL} channel satisfying the ellipsoidal uncertainty model, namely \cite{6026260}, \cite{5164911}.
\begin{equation}
	\Vert \pmb{E}_{t,k}^{\frac{1}{2}} \Delta \pmb{h}_{t,k} \Vert \leq 1, \quad \forall k.
\end{equation}
We can re-write the constraint in \eqref{eq:constraint-2-w-csi} herein as 
 \begin{equation}
	p_k\pmb{u}_k^H \pmb{h}_{t,k}\pmb{h}^H_{t,k} \pmb{u}_k
	-
	\zeta^{\tt{UL}}
	\sum\limits_{\substack{k' = 1 \\ k' \neq k }}^K p_{k'} \pmb{u}_k^H \pmb{h}_{t,k'}\pmb{h}^H_{t,k'} \pmb{u}_k
	\geq  
	\zeta^{\tt{UL}}_k
		\Big( 
	\pmb{u}_k^H \pmb{C}\pmb{Q}\pmb{C}^H \pmb{u}_k + 
	\pmb{u}_k^H \pmb{R}_c \pmb{u}_k +
	\sigma_n^2 \pmb{u}_k^H\pmb{u}_k\Big)
\end{equation}
Now we find a deterministic lower-bound of the upper-bound in the above inequality by utilizing the following bounds in \cite{6026260}
	\begin{equation}
		p_k\pmb{u}_k^H \pmb{h}_{t,k}\pmb{h}^H_{t,k} \pmb{u}_k
		=
		p_k 
		\Vert
		(\widehat{\pmb{h}}_{t,k}
	+ 
	\Delta \pmb{h}_{t,k})^H \pmb{u}_k
		\Vert^2  
		\geq
		p_k
		\Big[ \max (		\Vert
		(\widehat{\pmb{h}}_{t,k})^H \pmb{u}_k
		\Vert -  \Vert\pmb{E}_{t,k}^{-\frac{1}{2}} \pmb{u}_k\Vert
		,0 )
		\Big]^2
	\end{equation}
	
	\begin{equation}
		p_{k'} \pmb{u}_k^H \pmb{h}_{t,k'}\pmb{h}^H_{t,k'} \pmb{u}_k
  =
  p_{k'} 
  \Vert
		(\widehat{\pmb{h}}_{t,k'}
	+ 
	\Delta \pmb{h}_{t,k'})^H \pmb{u}_k
		\Vert^2
		\leq 
		p_{k'}
		\Big[
		\Vert
		\widehat{\pmb{h}}_{t,k'}^H \pmb{u}_k
		\Vert 
		+
		\Vert \pmb{E}_{t,k'}^{-\frac{1}{2}} \pmb{u}_k\Vert
		 \Big]^2
	\end{equation}
Combining the above two constraints, we have that
\begin{equation}
\label{eq:imperfect-csi-constraint-2}
	p_k f_{0,k}(\pmb{u}_k) - \zeta_k^{\tt{UL}}
	\sum\limits_{\substack{ k' \neq k }}
p_{k'}
f_{1,k'}(\pmb{u}_k)
\geq 
f_k(\pmb{V},\pmb{W},\pmb{u}_k), \forall k,
\end{equation}
where
\begin{align}
	f_{0,k}(\pmb{u}_k) &= 
	\big(		\Vert
		\widehat{\pmb{h}}_{t,k}^H \pmb{u}_k
		\Vert - \Vert\pmb{E}_{t,k}^{-\frac{1}{2}} \pmb{u}_k\Vert \big)^2, \\
	f_{1,k'}(\pmb{u}_k) &= \big(		\Vert
		(\widehat{\pmb{h}}_{t,k'})^H \pmb{u}_k
		\Vert + \Vert\pmb{E}_{t,k'}^{-\frac{1}{2}} \pmb{u}_k\Vert \big)^2, \\
	f_k(\pmb{V},\pmb{W},\pmb{u}_k) &=
		\zeta_k^{\tt{UL}}
		\big( 
	\pmb{u}_k^H \pmb{C}\pmb{Q}\pmb{C}^H \pmb{u}_k + 
	\pmb{u}_k^H \pmb{R}_c \pmb{u}_k +
	\sigma_n^2 \pmb{u}_k^H\pmb{u}_k\big)	.	
\end{align}
%% Constraint 3
The third constraint of problem \eqref{eq:problem1_1} of the updated manuscript is
\begin{equation}
\label{eq:constraint-3-w-csi}
	\SINR_{p,\tt{DFRC}}^{\tt{Eve}}
	=
	\frac
	{\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)}
	{\sum\limits_{\substack{k = 1  }}^K p_k \vert g_{k,p} \vert^2 + 
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2 }
	 \leq  \zeta_{p,\tt{DFRC}}^{\tt{Eve}}
\end{equation}
where in the presence of imperfect-\ac{CSI} we have that 
\begin{equation}
\label{eq:uncertain-gkp}
	g_{k,p}
	=
	\widehat{g}_{k,p}
	+ 
	\Delta g_{k,p}, \quad \forall k = 1 \ldots K, \quad \forall p = 1 \ldots P
\end{equation}
and we assume that 
\begin{equation}
	\Vert \Delta g_{k,p} \Vert \leq \epsilon_{k,p}, \quad \forall k,p.	
\end{equation}
We can re-write the above constraint in equation \eqref{eq:constraint-3-w-csi} herein as 
\begin{equation}
\label{constraint-3-rewritten}
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)
	-
	\zeta_{p,\tt{DFRC}}^{\tt{Eve}}
	\sum\limits_{\substack{k = 1  }}^K p_k \vert g_{k,p} \vert^2 
	\leq
	\zeta_{p,\tt{DFRC}}^{\tt{Eve}}
	\Big(
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2
	\Big)
\end{equation}
where we can bound the \ac{CSI} as 
	\begin{equation}
		p_{k} \vert g_{k,p} \vert^2
		=
		p_{k} \vert  \widehat{g}_{k,p} +  \Delta g_{k,p} \vert^2
		\geq 
		p_{k} 
		\Big[
		\vert \widehat{g}_{k,p} \vert - \epsilon_{k,p}
		\Big]^2
	\end{equation}	
Hence utilizing the above bound as an upper bound on the lower bound in \eqref{constraint-3-rewritten}, we have
%\begin{equation}
%	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)
%	-
%	\zeta_{p,\tt{DFRC}}^{\tt{Eve}}
%	\sum\limits_{\substack{k = 1  }}^K p_k 
%	(		\vert \widehat{g}_{k,p} \vert
%	-
%	 \epsilon_{k,p} )^2
%	\leq
%	\zeta_{p,\tt{DFRC}}^{\tt{Eve}}
%	\Big(
%	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
%	 + \sigma_p^2
%	\Big)
%\end{equation}
%This constraint corresponds to constraint \eqref{eq:imperfect-csi-constraint-3} in the updated manuscript, which has been re-written in a much more compact form.
%
%
%
%
%
%In a similar spirit, the third constraint in \eqref{eq:problem1_1} accounting for imperfect \ac{CSI} on $g_{k,p}$ for all $k,p$ can be written as
\begin{equation}
\label{eq:imperfect-csi-constraint-3}
\frac{1}{\zeta_{p,\tt{DFRC}}^{\tt{Eve}}}
	\phi_{0,p}(\pmb{V}) 
	-
	\sum_k
	p_k
	(		\vert \widehat{g}_{k,p} \vert
	-
	 \epsilon_{k,p} )^2
	\leq 
	\phi_{p}(\pmb{W}), \forall p,
\end{equation}
where
\begin{align}
	\phi_{0,p}(\pmb{V})  &= \vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)\\
	\phi_{p}(\pmb{W}) &= 
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2.
\end{align}
%% Constraint 4
Similarly, the fourth constraint in problem \eqref{eq:problem1_1} of the updated manuscript in the presence of imperfect \ac{CSI} on $g_{k,p}$, $\forall k,p$ is expressed as
\begin{equation}
\label{eq:imperfect-csi-constraint-4}
\frac{1}{\zeta_{p,k}^{\tt{Eve}}}
p_k
 (\vert \widehat{g}_{k,p} \vert
+
\epsilon_{k,p} )^2
 -
 \sum\nolimits_{k' \neq k } p_{k'} (		\vert \widehat{g}_{k',p} \vert
-
\epsilon_{k',p} )^2
 \leq 
	 \phi_{p}(\pmb{Q}).
\end{equation}
%% Optimization problem
The \ac{FD} \ac{ISAC} power minimization with imperfect-\ac{CSI} optimization problem can now be written as
\begin{equation}
 \label{eq:problem1_1_imperfect_csi}
\begin{aligned}
(\mathcal{P}^{\tt{robust}}):
\begin{cases}
\min\limits_{\lbrace \substack{ \pmb{U},
									 \pmb{V},  
									 \pmb{W}, 
									  \pmb{p},
									  \pmb{s} }  \rbrace}&   \trace(\pmb{VV}^H) + \trace(\pmb{W}) + \pmb{1}^T \pmb{p} \\
\textrm{s.t.}
 &  \eqref{eq:imperfect-csi-constraint-1},
 	\eqref{eq:imperfect-csi-constraint-2},
 	\eqref{eq:imperfect-csi-constraint-3},
 	\eqref{eq:imperfect-csi-constraint-4}, \\
& \ISMR \leq \ISMR_{\tt{max}} , \\
 & \pmb{W} \succeq \pmb{0}, \  \pmb{p} \succeq \pmb{0}, \pmb{s} \succeq \pmb{0}, \\
\end{cases}
\end{aligned}
\end{equation}
Due to the non-convexity of the problem, we design a \ac{BCCD} method due to the decoupled nature of some constraints in this formulation, which further allows us to devise an iterative \ac{BCCD} algorithm over the beamformers, slack variables and power levels. 
% V,W,s
To this end, we first solve the problem with respect to $\pmb{V},\pmb{W},\pmb{s}$ by fixing $\pmb{p}$ and $\pmb{U}$. Therefore, given $\pmb{p}^{(m)}$ and $\pmb{U}^{(m)}$ at iteration $m$, constraints 
\eqref{eq:imperfect-csi-constraint-1},
\eqref{eq:imperfect-csi-constraint-2},
 	\eqref{eq:imperfect-csi-constraint-3}, and 
 	\eqref{eq:imperfect-csi-constraint-4} become 
 	
\begin{equation}
\label{eq:imperfect-csi-constraint-1-fix-p}
	\begin{bmatrix}
		\widehat{\pmb{h}}_{r,\ell}^H 
		\pmb{Q}_\ell 
		\widehat{\pmb{h}}_{r,\ell}
		-
		\zeta_{\ell}^{\tt{DL}}
		\sigma_{\ell}^2
		-\zeta_{\ell}^{\tt{DL}}\sum\limits_{\substack{k = 1  }}^K p_k^{(m)} \vert q_{k,\ell} \vert^2 
		-
		s_\ell &
		\widehat{\pmb{h}}_{r,\ell}^H 
		\pmb{Q}_\ell  \\
\pmb{Q}_\ell 
		\widehat{\pmb{h}}_{r,\ell} &
		\pmb{Q}_\ell  + s_\ell \pmb{E}_{r,\ell}	
	\end{bmatrix}
	\succeq \pmb{0},
\end{equation} 	
\begin{equation}
\label{eq:imperfect-csi-constraint-2-fix-pU}
	p_k^{(m)} f_{0,k}(\pmb{u}_k^{(m)}) - \zeta_k^{\tt{UL}}
	\sum\limits_{\substack{ k' \neq k }}
p_{k'}^{(m)}
f_{1,k'}(\pmb{u}_k^{(m)})
\geq 
f_k(\pmb{V},\pmb{W},\pmb{u}_k^{(m)}),
\end{equation}
\begin{equation}
\label{eq:imperfect-csi-constraint-3-fix-pU}
\frac{1}{\zeta_{p,\tt{DFRC}}^{\tt{Eve}}}
	\phi_{0,p}(\pmb{V}) 
	-
	\sum\nolimits_k
	p_k^{(m)}
	(		\vert \widehat{g}_{k,p} \vert
	-
	 \epsilon_{k,p} )^2
	\leq 
	\phi_{p}(\pmb{W}),
\end{equation}
and
\begin{equation}
\label{eq:imperfect-csi-constraint-4-fix-pU}
\frac{1}{\zeta_{p,k}^{\tt{Eve}}}
p_k^{(m)}
 (\vert \widehat{g}_{k,p} \vert
+
\epsilon_{k,p} )^2
 -
 \sum\limits_{k' \neq k } p_{k'}^{(m)} (		\vert \widehat{g}_{k',p} \vert
-
\epsilon_{k',p} )^2
 \leq 
	 \phi_{p}(\pmb{Q}),
\end{equation} 	
respectively. Hence, the first sub-problem to solve is 
\begin{equation}
 \label{eq:problem1_1_imperfect_csi_problem_1}
\begin{aligned}
(\mathcal{P}^{\tt{robust}}_1):
\begin{cases}
\min\limits_{\lbrace \substack{\pmb{V},  
									 \pmb{W}, 
									  \pmb{s} }  \rbrace}&   \trace(\pmb{VV}^H) + \trace(\pmb{W})  \\
\textrm{s.t.}
 &  \eqref{eq:imperfect-csi-constraint-1-fix-p},
 	\eqref{eq:imperfect-csi-constraint-2-fix-pU},
 	\eqref{eq:imperfect-csi-constraint-3-fix-pU},
 	\eqref{eq:imperfect-csi-constraint-4-fix-pU}, \\
& \ISMR \leq \ISMR_{\tt{max}} , \\
 & \pmb{W} \succeq \pmb{0}, \pmb{s} \succeq \pmb{0}, \\
\end{cases}
\end{aligned}
\end{equation}
% p
After solving $(\mathcal{P}^{\tt{robust}}_1)$ to obtain $\pmb{V}^{(m+1)},  
									 \pmb{W}^{(m+1)}$, and  $\pmb{s}^{(m+1)}$, we now solve \eqref{eq:problem1_1_imperfect_csi} by fixing $\pmb{U}, \pmb{V},\pmb{W}$ and $\pmb{s}$ to $\pmb{U}^{(m)}, \pmb{V}^{(m+1)},\pmb{W}^{(m+1)}$ and $\pmb{s}^{(m+1)}$, respectively. 
This means that constraints 
\eqref{eq:imperfect-csi-constraint-1},
\eqref{eq:imperfect-csi-constraint-2},
 	\eqref{eq:imperfect-csi-constraint-3}, and 
 	\eqref{eq:imperfect-csi-constraint-4} are now 
 	
\begin{equation}
\label{eq:imperfect-csi-constraint-1-fix-UVW}
	\begin{bmatrix}
		\widehat{\pmb{h}}_{r,\ell}^H 
		\pmb{Q}_\ell^{(m+1)} 
		\widehat{\pmb{h}}_{r,\ell}
		-
		\zeta_{\ell}^{\tt{DL}}
		\sigma_{\ell}^2
		-\zeta_{\ell}^{\tt{DL}}\sum\limits_{\substack{k = 1  }}^K p_k \vert q_{k,\ell} \vert^2 
		-
		s_\ell^{(m+1)} &
		\widehat{\pmb{h}}_{r,\ell}^H 
		\pmb{Q}_\ell^{(m+1)}  \\
\pmb{Q}_\ell^{(m+1)} 
		\widehat{\pmb{h}}_{r,\ell} &
		\pmb{Q}_\ell^{(m+1)}  + s_\ell^{(m+1)} \pmb{E}_{r,\ell}	
	\end{bmatrix}
	\succeq \pmb{0},
\end{equation} 	
where $\pmb{Q}_\ell^{(m+1)} = \pmb{V}_\ell^{(m+1)} - \zeta_{\ell}^{\tt{DL}} \pmb{W}^{(m+1)} - \zeta_{\ell}^{\tt{DL}} \sum\nolimits_{\ell' \neq \ell} \pmb{V}_{\ell'}^{(m+1)}$, $\forall \ell$ and
\begin{equation}
\label{eq:imperfect-csi-constraint-2-fix-UVW}
	p_k f_{0,k}(\pmb{u}_k^{(m)}) - \zeta_k^{\tt{UL}}
	\sum\limits_{\substack{ k' \neq k }}
p_{k'}
f_{1,k'}(\pmb{u}_k^{(m)})
\geq 
f_k(\pmb{V}^{(m+1)},\pmb{W}^{(m+1)},\pmb{u}_k^{(m)}),
\end{equation}
\begin{equation}
\label{eq:imperfect-csi-constraint-3-fix-UVW}
\frac{1}{\zeta_{p,\tt{DFRC}}^{\tt{Eve}}}
	\phi_{0,p}(\pmb{V}^{(m+1)}) 
	-
	\sum\nolimits_k
	p_k
	(		\vert \widehat{g}_{k,p} \vert
	-
	 \epsilon_{k,p} )^2
	\leq 
	\phi_{p}(\pmb{W}^{(m+1)}),
\end{equation}
and
\begin{equation}
\label{eq:imperfect-csi-constraint-4-fix-UVW}
\frac{1}{\zeta_{p,k}^{\tt{Eve}}}
p_k
 (\vert \widehat{g}_{k,p} \vert
+
\epsilon_{k,p} )^2
 -
 \sum\limits_{k' \neq k } p_{k'}(		\vert \widehat{g}_{k',p} \vert
-
\epsilon_{k',p} )^2
 \leq 
	 \phi_{p}(\pmb{Q}^{(m+1)}),
\end{equation} 	
respectively.
Therefore, we now have the following	 sub-problem to solve
\begin{equation}
 \label{eq:problem1_1_imperfect_csi_problem_2}
\begin{aligned}
(\mathcal{P}^{\tt{robust}}_2):
\begin{cases}
\min\limits_{\pmb{p} }& \pmb{1}^T \pmb{p} \\
\textrm{s.t.}
 & \eqref{eq:imperfect-csi-constraint-1-fix-UVW},
  \eqref{eq:imperfect-csi-constraint-2-fix-UVW},
 	\eqref{eq:imperfect-csi-constraint-3-fix-UVW},
 	\eqref{eq:imperfect-csi-constraint-4-fix-UVW}, \\
 & \pmb{p} \succeq \pmb{0}, \\
\end{cases}
\end{aligned}
\end{equation}						 
% u
Finally, solving $(\mathcal{P}^{\tt{robust}}_2)$ to obtain $ \pmb{p}^{(m+1)}$, we can now update the beamformers $\pmb{U}^{(m+1)}$ following equation \eqref{eq:uk-in-closed-form} of the updated manuscript, by utilizing the available \ac{CSI} $\widehat{\pmb{h}}_{t,k}$ and the latest updates $\pmb{p}^{(m+1)}$ and $\pmb{Q}^{(m+1)}$.
We now summarize the steps of the \ac{BCCD} method for \ac{FD} \ac{ISAC} power minimization with imperfect \ac{CSI}.
First, the \ac{BCCD} method aims at first solving $(\mathcal{P}^{\tt{robust}}_1)$ in \eqref{eq:problem1_1_imperfect_csi_problem_1} to obtain $\pmb{V}^{(m+1)},  
									 \pmb{W}^{(m+1)}$, and  $\pmb{s}^{(m+1)}$.
Then, the \ac{BCCD} solves $(\mathcal{P}^{\tt{robust}}_2)$ in \eqref{eq:problem1_1_imperfect_csi_problem_2} to obtain $\pmb{p}^{(m+1)}$.
Finally, we update $\pmb{U}^{(m+1)}$ using equation \eqref{eq:uk-in-closed-form} of the updated manuscript.
The \ac{BCCD} iterates over the three sub-problems until convergence.









==> sections/optimization02.tex <==
In the second problem, we deal with
\begin{equation}
 \label{eq:problem2_1}
\begin{aligned}
(\mathcal{P}_2):
\begin{cases}
\max\limits_{\lbrace \substack{ \pmb{U},
									 \pmb{V},  
									 \pmb{W}, 
									  \pmb{p} }  \rbrace}&  \SR_{\tt{
									  DL}} \\
\textrm{s.t.}
 &  \SR_{\tt{UL}} \geq R, \\
 & \trace(\pmb{VV}^H) + \trace(\pmb{W}) + \pmb{1}^T \pmb{p} \leq P_b, \\
& \ISMR \leq \ISMR_{\tt{max}} , \\
& \pmb{W} \succeq \pmb{0},  \ \pmb{p} \succeq \pmb{0}   \\\end{cases}
\end{aligned}
\end{equation}
%%% Replacing the expressions
\begin{equation}
 \label{eq:problem2_2}
\begin{aligned}
(\mathcal{P}_2):
\begin{cases}
\max\limits_{\lbrace \substack{ \pmb{U},
									 \pmb{V},  
									 \pmb{W}, 
									  \pmb{p} }  \rbrace}&  \min_{\ell,p}
	\Big[
	\log_2(1+\SINR_{\ell}^{\tt{DL}})
	-
	\log_2(1+\SINR_{p,\tt{DFRC}}^{\tt{Eve}})
	\Big] \\
\textrm{s.t.}
 &  \min_{k,p}
	\Big[
	\log_2(1+\SINR_{k}^{\tt{UL}})
	-
	\log_2(1+\SINR_{p,k}^{\tt{Eve}})
	\Big] \geq R, \\
 & \trace(\pmb{VV}^H) + \trace(\pmb{W}) + \pmb{1}^T \pmb{p} \leq P_b, \\
& \ISMR \leq \ISMR_{\tt{max}} , \\
& \pmb{W} \succeq \pmb{0},  \ \pmb{p} \succeq \pmb{0}   \\\end{cases}
\end{aligned}
\end{equation}
%% 

\begin{equation}
 \label{eq:problem2_3}
\begin{aligned}
(\mathcal{P}_2):
\begin{cases}
\max\limits_{\Bigg\lbrace \substack{ \pmb{U}\\
									 \pmb{V} \\ 
									 \pmb{W} \\
									  \pmb{p} \\ \theta } \Bigg\rbrace}&  
									  \min_{\ell}
	\Big[
	\log_2(1+\SINR_{\ell}^{\tt{DL}})
	-
	\log_2(1+\theta)
	\Big] \\
\textrm{s.t.}
& \frac
	{\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{VV}^H\pmb{a}_{N_T}(\theta_p)}
	{\sum\limits_{\substack{k = 1  }}^K p_k \vert g_{k,p} \vert^2 + 
	\vert \alpha_p \vert^2 \pmb{a}_{N_T}^H(\theta_p)\pmb{W}\pmb{a}_{N_T}(\theta_p)
	 + \sigma_p^2 } \leq \theta, \ \forall p, \\ 
 &  \min_{k,p}
	\Big[
	\log_2(1+\SINR_{k}^{\tt{UL}})
	-
	\log_2(1+\SINR_{p,k}^{\tt{Eve}})
	\Big] \geq R, \\
 & \trace(\pmb{VV}^H) + \trace(\pmb{W}) + \pmb{1}^T \pmb{p} \leq P_b, \\
& \ISMR \leq \ISMR_{\tt{max}} , \\
& \pmb{W} \succeq \pmb{0},  \ \pmb{p} \succeq \pmb{0}   \\\end{cases}
\end{aligned}
\end{equation}



